Fast Few-Shot Classification by Few-Iteration Meta-Learning

Autonomous agents interacting with the real world need to learn new concepts efficiently and reliably. This requires learning in a low-data regime, which is a highly challenging problem. We address this task by introducing a fast optimization-based meta-learning method for few-shot classification. It consists of an embedding network, providing a general representation of the image, and a base learner module. The latter learns a linear classifier during the inference through an unrolled optimization procedure. We design an inner learning objective composed of (i) a robust classification loss on the support set and (ii) an entropy loss, allowing transductive learning from unlabeled query samples. By employing an efficient initialization module and a Steepest Descent based optimization algorithm, our base learner predicts a powerful classifier within only a few iterations. Further, our strategy enables important aspects of the base learner objective to be learned during meta-training. To the best of our knowledge, this work is the first to integrate both induction and transduction into the base learner in an optimization-based meta-learning framework. We perform a comprehensive experimental analysis, demonstrating the speed and effectiveness of our approach on four few-shot classification datasets. The Code is available at \href{https://github.com/4rdhendu/FIML}{\textcolor{blue}{https://github.com/4rdhendu/FIML}}.

==> broad_impact.tex <==
Here, we discuss the societal and ethical aspects of the proposed approach. Our approach falls into the broad category of 'learning to learn' or meta-learning algorithms. Meta-learning algorithms generalise AI to scenarios with minimum amount of training data. There are a multitude of areas where meta-learning algorithms can find application \eg detection and diagnosis of rare diseases, continuous learning in autonomous vehicles, and many more. 
% Alet \etal~\cite{curiosity} call meta-learning algorithms curious. The evolving nature of these algorithm's makes their long term behaviour difficult to control hence, it is pivotal to modulate and regulate meta-learning algorithm's by drawing strict guidelines for employing them. 
It can be difficult to formulate specifications for a system that evolves with experience. These systems therefore must be evaluated at regular intervals throughout the period of use, \eg keeping a track of the accidents involving autonomous vehicles. It is necessary to guard meta-learning algorithms from biases induced due to the experiences they have had. Further, making them more interpretable and regulating these systems well promise to benefit many facets of human life.  


